CompAct: Compressing Retrieved Documents Actively for Question Answering

Retrieval-augmented generation supports language models to strengthen their factual groundings by providing external contexts. However, language models often face challenges when given extensive information, diminishing their effectiveness in solving questions. Context compression tackles this issue by filtering out irrelevant information, but current methods still struggle in realistic scenarios where crucial information cannot be captured with a single-step approach. To overcome this limitation, we introduce CompAct, a novel framework that employs an active strategy to condense extensive documents without losing key information. Our experiments demonstrate that CompAct brings significant improvements in both performance and compression rate on multi-hop question-answering benchmarks. CompAct flexibly operates as a cost-efficient plug-in module with various off-the-shelf retrievers or readers, achieving exceptionally high compression rates (47x).

==> figures/Contriever_plot.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=.78\columnwidth]{figures/Contriever.pdf}
\caption{
Performance of HotpotQA using Contriever.
}
\label{fig:contriever}
\vspace{-0.3cm}
\end{figure}

==> figures/llama3_8b_plot.tex <==
% \begin{figure}[]
% \centering
% \includegraphics[width=.98\columnwidth]{figures/llama3_8b.pdf}
% \caption{
% Performance of HotpotQA with different top-$k$ documents. 
% We set the reader as LLaMA3-8B.
% }
% \label{fig:reader_llama3_8b}
% \end{figure}

==> tables/inference_hotpot.tex <==
\begin{table}[t]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Methods} & \textbf{Compress} & \textbf{Read} & \textbf{Total} / \textbf{Throughput}  & \textbf{F1} \\ \midrule
No Documents & -    & 1.5m & 1.5m / 5.58 & 31.7\\ 
Raw Documents  & -    & 11.5m & 11.5m / 0.72 & 42.5\\ 
RECOMP    & \textbf{2.1m} & 1.9m & \textbf{4.0m} / \textbf{2.10} & 41.5\\ 
LongLLMLingua  & 32.3m & 3.3m & 35.6m / 0.23 & 35.5\\
\midrule
% \begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (5 docs)\end{tabular}  & 1.4m & 178.7m & 180.1m & 0.05 & 47.3 \\ 
\begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (5 docs)\end{tabular}  & 147.9m & \textbf{1.5m} & 149.3m / 0.06 & \textbf{47.3} \\ 
% \begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (10 docs)\end{tabular} & 1.9m & 92.9m & 94.8m & 0.09 & 45.4 \\ \bottomrule
\begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (10 docs)\end{tabular} & 77.2m & 1.9m & 79.1m / 0.11 & 45.4 \\ \bottomrule
\end{tabular}}}{}
\caption{
% We measure inference GPU time (read), compression GPU time, total GPU time (inference + compression), and throughput (examples per second).
We measure GPU time taken to compress source documents and read the compressed texts.
Also, we report the throughput (examples per second) and the corresponding end performance (F1) to compare the benefit of \textsc{CompAct} with other baselines.
% Our iterative inference lets us consider the trade-off between massive inference time and high performance (compression rate and end QA performance).
}
\label{tab:latency_hotpot}
\vspace{-0.3cm}
\end{table}


==> tables/inference_nq.tex <==
\begin{table}[t]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Baselines}    & \begin{tabular}[c]{@{}c@{}}\textbf{Inference}\\ \textbf{GPU Time}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Compression}\\ \textbf{GPU Time}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Total}\\ \textbf{GPU Time}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Throughput}\\ \textbf{(example/sec)}\end{tabular} & \textbf{F1}  \\ \midrule
No Documents & 1.9m  & - & 1.9m & 4.33 & 39.3 \\ 
Raw Documents   & 10.9m  & - & 10.9m & 0.76 & 52.1 \\ 
RECOMP & 4.2m  &  1.6m   & 5.7m & 1.45 & 46.6 \\ 
LongLLMLingua   & 3.6m  & 31.4m   & 35.0m & 0.24 & 42.4 \\ 
\midrule
\begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (5 docs) \end{tabular}  & 2.2m  & 136.5m & 138.7m & 0.06 & 52.8 \\ 
\begin{tabular}[c]{@{}l@{}}\textsc{CompAct} (10 docs) \end{tabular} & 2.2m & 80.0m & 82.2m & 0.10 & 51.2 \\ \bottomrule
\end{tabular}}}{}
\caption{Inference time for NQ dataset. Our iterative inference lets us consider the trade-off between massive inference time and high performance (compression rate and end QA performance).}
\label{tab:latency_nq}
\end{table}

==> tables/reader_agnostic_top10.tex <==
\begin{table}[]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{Baselines}} & \multicolumn{3}{c}{\textbf{Reader LLMs}} \\ \cmidrule{2-4} 
 &  \multicolumn{1}{c}{\textbf{LLaMA2-13B}} & \multicolumn{1}{c}{\textbf{LLaMA3-8B}} & \textbf{GPT-3.5-Turbo} \\ \midrule
Gold Documents   & 49.4 & 49.4 & 48.7    \\ 
Raw Documents    & 39.8 & 41.3 & 45.5    \\       \midrule
RECOMP      & 40.0 & 39.3 & 42.0    \\    
LongLLMLingua    & 35.0 & 35.7 & 37.2    \\     
CompAct (Ours)   & 46.9 & 46.1 & 45.2    \\       \bottomrule
\end{tabular}}}{}
\caption{
\textcolor{redcolor}{Top-10 results, our \textsc{CompAct} works well regardless of reader LLMs}}
\label{table:generalize_top40}
\end{table}

==> tables/reader_agnostic_top20.tex <==
\begin{table}[]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{Baselines}} & \multicolumn{3}{c}{\textbf{Reader LLMs}} \\ \cmidrule{2-4} 
 &  \multicolumn{1}{c}{\textbf{LLaMA2-13B}} & \multicolumn{1}{c}{\textbf{LLaMA3-8B}} & \textbf{GPT-3.5-Turbo} \\ \midrule
Gold Documents   & 51.0 & 51.0 & 51.5    \\ 
Raw Documents    & 33.2 & 39.8 & 46.6    \\       \midrule
RECOMP      & 40.9 & 39.5 & 40.5    \\    
LongLLMLingua    & 34.1 & 35.6 & 35.2    \\     
CompAct (Ours)   & 48.0 & 45.8 & 47.0    \\       \bottomrule
\end{tabular}}}{}
\caption{
\textcolor{redcolor}{Top-20 results, our \textsc{CompAct} works well regardless of reader LLMs}}
\label{table:generalize_top40}
\end{table}

==> tables/reader_agnostic_top30.tex <==
\begin{table}[]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{l cccc}
\toprule
\multirow{2}{*}{\textbf{Baselines}} & \multicolumn{4}{c}{\textbf{Reader LLMs}} \\ \cmidrule{2-5} 
 & \multicolumn{1}{c}{\textbf{LLaMA2-7B}} & \multicolumn{1}{c}{\textbf{LLaMA2-13B}} & \multicolumn{1}{c}{\textbf{LLaMA3-8B}} & \textbf{GPT-3.5-Turbo} \\ \midrule
Gold Documents   & \multicolumn{1}{c}{49.6} & 51.2 & \multicolumn{1}{c}{52.4} & 53.2     \\ 
Raw Documents    & \multicolumn{1}{c}{32.4} & \multicolumn{1}{c}{31.2}  & \multicolumn{1}{c}{40.2} & 44.1     \\ \midrule
RECOMP      & \multicolumn{1}{c}{34.1} & \multicolumn{1}{c}{39.7} & \multicolumn{1}{c}{38.5} &  \multicolumn{1}{c}{39.4}   \\ 
LongLLMLingua    & \multicolumn{1}{c}{30.9} & \multicolumn{1}{c}{32.9} & \multicolumn{1}{c}{35.5} & \multicolumn{1}{c}{39.0}    \\ 
CompAct (Ours)   & \multicolumn{1}{c}{\textbf{45.0}} & \multicolumn{1}{c}{\textbf{47.1}}  & \multicolumn{1}{c}{\textbf{46.9}} & \textbf{48.1}     \\ \bottomrule
\end{tabular}}}{}
\caption{
\textcolor{redcolor}{Top-30 results, our \textsc{CompAct} works well regardless of reader LLMs}}
\label{table:generalize}
\end{table}

==> tables/reader_agnostic_top40.tex <==
\begin{table}[]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{Baselines}} & \multicolumn{3}{c}{\textbf{Reader LLMs}} \\ \cmidrule{2-4} 
 &  \multicolumn{1}{c}{\textbf{LLaMA2-13B}} & \multicolumn{1}{c}{\textbf{LLaMA3-8B}} & \textbf{GPT-3.5-Turbo} \\ \midrule
Gold Documents   & 53.6 & 53.6 &  54.3   \\ 
Raw Documents    & 37.7 & 37.7 &  43.7   \\       \midrule
RECOMP      & 40.0 & 39.5 & 39.6  \\    
LongLLMLingua    & 33.3 & 34.4 &  36.9   \\     
CompAct (Ours)   & 47.5 & 47.5 & 46.8    \\       \bottomrule
\end{tabular}}}{}
\caption{
\textcolor{redcolor}{Top-40 results, our \textsc{CompAct} works well regardless of reader LLMs}}
\label{table:generalize_top40}
\end{table}

==> tables/reader_agnostic_top5.tex <==
\begin{table}[]
\centering
{\resizebox{0.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{\textbf{Baselines}} & \multicolumn{3}{c}{\textbf{Reader LLMs}} \\ \cmidrule{2-4} 
 &  \multicolumn{1}{c}{\textbf{LLaMA2-13B}} & \multicolumn{1}{c}{\textbf{LLaMA3-8B}} & \textbf{GPT-3.5-Turbo} \\ \midrule
Gold Documents   & 47.3 & 47.3 & 46.8    \\ 
Raw Documents    & 41.4 & 43.6 & 44.4    \\       \midrule
RECOMP      & 41.9 & 40.0 & 43.4    \\    
LongLLMLingua    & 35.9 & 33.9 & 36.1    \\     
CompAct (Ours)   & 46.5 & 45.1 & 44.6    \\       \bottomrule
\end{tabular}}}{}
\caption{
\textcolor{redcolor}{Top-5 results, our \textsc{CompAct} works well regardless of reader LLMs}}
\label{table:generalize_top40}
\end{table}
